LB-SimTSC: An Efficient Similarity-Aware Graph Neural Network for Semi-Supervised Time Series Classification

Time series classification is an important data mining task that has received a lot of interest in the past two decades. Due to the label scarcity in practice, semi-supervised time series classification with only a few labeled samples has become popular. Recently, Similarity-aware Time Series Classification (SimTSC) is proposed to address this problem by using a graph neural network classification model on the graph generated from pairwise Dynamic Time Warping (DTW) distance of batch data. It shows excellent accuracy and outperforms state-of-the-art deep learning models in several few-label settings. However, since SimTSC relies on pairwise DTW distances, the quadratic complexity of DTW limits its usability to only reasonably sized datasets. To address this challenge, we propose a new efficient semi-supervised time series classification technique, LB-SimTSC, with a new graph construction module. Instead of using DTW, we propose to utilize a lower bound of DTW, LB_Keogh, to approximate the dissimilarity between instances in linear time, while retaining the relative proximity relationships one would have obtained via computing DTW. We construct the pairwise distance matrix using LB_Keogh and build a graph for the graph neural network. We apply this approach to the ten largest datasets from the well-known UCR time series classification archive. The results demonstrate that this approach can be up to 104x faster than SimTSC when constructing the graph on large datasets without significantly decreasing classification accuracy.

==> tmp.tex <==
\section{Related Work}

\subsection{Lower bounding measure}
Lower bounding measure is introduced to speed up time series similarity search. Numerous non-trivial lower bounding measures have been studied~\cite{yi1998efficient,kim2001index,keogh2005exact,webb2021tight,lemire2009faster,shen2018accelerating,tan2019elastic}. Among them, LB\_Keogh~\cite{keogh2005exact} is one of the most tightness and fastest ($O(l)$) lower-bound DTW algorithm. The authors use sliding windows to calculate upper and lower bounds as the envelope for subsequences of candidate time series, and use ED to calculate the distance of the target time series beyond the envelope. We will describe LB\_Keogh in detail in Section~\ref{preliminaries}.

\subsection{Time series few-shot learning}
In TSC, many deep learning models have been proven to work well for TSC~\cite{ismail2020inceptiontime,karim2017lstm,li2021shapenet,zhang2020tapnet,wang2017time}, but only few researchers study time series few-shot learning.  Time series attentional prototype network (TapNet)~\cite{zhang2020tapnet} learns prototype for each class and take semi-supervised learning into account. SimTSC~\cite{zha2022towards} combines similarity measure and GNN and is proved its effectiveness on data with very few labels. But its reliance on DTW makes it inefficient for large datasets.

Our paper studies time series few-shot learning while considering the effectiveness of training on large datasets.
